Dynamic Legged Manipulation of a Ball Through Multi-Contact Optimization

The feet of robots are typically used to design locomotion strategies, such as balancing, walking, and running. However, they also have great potential to perform manipulation tasks. In this paper, we propose a model predictive control (MPC) framework for a quadrupedal robot to dynamically balance on a ball and simultaneously manipulate it to follow various trajectories such as straight lines, sinusoids, circles and in-place turning. We numerically validate our controller on the Mini Cheetah robot using different gaits including trotting, bounding, and pronking on the ball.

==> problem_bak.tex <==
\section{Background}
\label{sec:problem}

\subsection{MIT Mini Cheetah Controller}
\bike{rewrite this sub-section to introduce MPC and WBIC for Mini Cheetah.}
The MIT Mini Cheetah \cite{kim2019highly} has advanced dynamic locomotion capabilities with its control strategy combining a model predictive controller (MPC) and a whole-body impulse controller (WBIC). 
The low-frequency, simple-model and long-horizon MPC complements the high-frequency, full-model and short-horizon WBIC.
Specifically, the MPC plans the contact force of a full gait cycle with a simple lumped mass model to track the desired body trajectory.
In this paper, our goal is to enable a quadrupedal robot dynamically manipulate a ball like balancing on it.
Specifically, our robot is required to manipulate a ball to track a given trajectory. In order to exploit the hardware capabilities of legged systems, the non-contact phases need to be considered in the locomotion problem.
One of the state of the art \cite{kim2019highly} proposes a method where a control framework of two cascaded simpler controllers are applied to the locomotion optimization.
The first controller is a full gait cycle of locomotion using a model predictive controller (MPC) with a simple lumped mass model, followed by a whole-body impulse control (WBIC) which generates torque command through a PD control with respect to the desired joint position and velocity.
When this control framework is used on the robot to achieve the manipulation tasks, it is no longer robust to the perturbations from ball movement, since the manipulation of the ball changes the dynamics of the whole system.
Our algorithm adopts the control hierarchy in \cite{kim2019highly} and makes extensions, so that we could control the robot and the ball at the same time. We will discuss the algorithm of control design in Section \ref{sec:algorithm}. In this problem, we use a Mini Cheetah \cite{katz2019mini, kim2019highly, bledt2018contact} as our quadrupedal robot model.
We also try different locomotion gaits to validate our control strategy, shown in Fig.~\ref{fig:gait}.
The robot is able to perform manipulation tasks using trotting, bounding, and pronking gait.

\begin{figure}
    \centering
    \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\linewidth]{images/trot00.jpg}
      \caption{Trotting gait}
      \label{fig:trotting}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\linewidth]{images/bound00.jpg}
      \caption{Bounding gait}
      \label{fig:bounding}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\linewidth]{images/pronk00.jpg}
      \caption{Pronking gait}
      \label{pronking}
    \end{subfigure}
    \caption{Mini Cheetah manipulating a ball using different gaits: (a) trotting, (b) bounding, and (c) pronking.
    % \ayush{This figure is not very illustrative of the gait type - all figures seem to be of the cheetah standing. We should either remove this or have a better figure.}
    The swing feet and their trajectories are denoted by brown (initial position), green (current position), and red (end position) spheres, while the stance feet are colored in blue. The red arrows show the reaction forces.
    }
    \label{fig:gait}
\end{figure}
